Retrieve and Copy: Scaling ASR Personalization to Large Catalogs

Personalization of automatic speech recognition (ASR) models is a widely studied topic because of its many practical applications. Most recently, attention-based contextual biasing techniques are used to improve the recognition of rare words and domain specific entities. However, due to performance constraints, the biasing is often limited to a few thousand entities, restricting real-world usability. To address this, we first propose a "Retrieve and Copy" mechanism to improve latency while retaining the accuracy even when scaled to a large catalog. We also propose a training strategy to overcome the degradation in recall at such scale due to an increased number of confusing entities. Overall, our approach achieves up to 6% more Word Error Rate reduction (WERR) and 3.6% absolute improvement in F1 when compared to a strong baseline. Our method also allows for large catalog sizes of up to 20K without significantly affecting WER and F1-scores, while achieving at least 20% inference speedup per acoustic frame.

==> f1_configs_latency_configs.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{f1_models_fullcatalog.png}
         \caption{}
         \label{fig:y equals x}
     \end{subfigure}%
     %\hfill
     \bigskip
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{f1_models_fullcatalog.png}
         \caption{}
         \label{fig:three sin x}
     \end{subfigure}%
     %\hfill
     \bigskip
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{f1_models_fullcatalog.png}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}%
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{f1_models_fullcatalog.png}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}%
     \bigskip
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{f1_models_fullcatalog.png}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}%
     \bigskip
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{f1_models_fullcatalog.png}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}%
        \caption{Three simple graphs}
        \label{fig:three graphs}
\end{figure*}

==> f1_configs_models.tex <==
\captionsetup{width=\columnwidth}
\begin{figure}
  \centering
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{f1_models_fullcatalog.png}
  \end{subfigure}
  \vspace{-1em}
  \begin{subfigure}{\columnwidth}
    \centering
  \includegraphics[width=\linewidth]{f1_models_faiss.png}
  \end{subfigure}
  \vspace{0.5em}
  \caption{\footnotesize{BASE vs BASE+CA vs BASE+CA+HN-FT: F1 without (left) and with retrieve (right) for varying catalogs.}}
  \label{fig:f1_models_configs}
\end{figure}

==> f1_faiss_latency_hyperparams.tex <==
\captionsetup{width=\columnwidth}
\begin{figure}[!htp]
  \centering
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{faiss_retrieval_accuracy.png}
  \end{subfigure}
  \vspace{-1em}
  \begin{subfigure}{\columnwidth}
    \centering
   \includegraphics[width=\linewidth]{faiss_latency.png}
  \end{subfigure}
  \vspace{0.5em}
  \caption{\footnotesize{Effect of number of entities retrieved by FAISS on retrieval accuracy and latency for BASE+CA model.}}
  \label{fig:f1_latency_hyperparams}
\end{figure}

==> f1_latency_configs.tex <==
\captionsetup{width=\columnwidth}
\begin{figure}[!htp]
  \centering
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{F1_configs.png}
  \end{subfigure}
  \vspace{-1em}
  \begin{subfigure}{\columnwidth}
    \centering
   \includegraphics[width=\linewidth]{Latency_configs.png}
  \end{subfigure}
  \vspace{0.5em}
  \caption{\footnotesize{Effect of FAISS Retrieval on F1 (left) and Latency (right) for varying catalogs for the BASE+CA model.}}
  \label{fig:f1_latency_configs}
\end{figure}

==> generic-dataset.tex <==
% \begin{table}[!htbp]\footnotesize
% \centering
% \setlength\tabcolsep{3.5pt}
% \begin{tabular}{ll|cc}
% \toprule
%   Model & Inference & WER & F1 \\
%   \hline
%   STREAM-BASE & N/A & 10.5 & 65.5 \\
%   \hline
%   \multirow{2}{*}{STREAM-ADAPT} & Full Catalog & 10.9 & 71.4 \\
%   & FAISS & 10.9 & 71.8\\
%   \hline
%   \multirow{2}{*}{STREAM-ADAPT-DISC} & Full Catalog & 11.3 & 73.3 \\
%   & FAISS & 11.4 & 73.3\\
%  \bottomrule
% \end{tabular}
% \caption{Performance of our models for the generic VoxPopuli dataset.}
% \label{tab:generic-dataset}
% \end{table}

==> model-architecture-overall.tex <==

% overall model architecture similar to 
% https://quip-amazon.com/v8TwA6D4hunk/Contextual-Biasing-with-Large-Catalogs-for-All-Neural-Lex-ASR#temp:C:UNHff73a51cdf7f4076996a6e2a3

==> varying-catalog-sizes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
% \begin{table*}[!htbp]
\centering
\begin{tabular}{|c|c|c|ccc|ccc|}
\hline
\multirow{2}{*}{MODEL} &
  \multirow{2}{*}{CATALOG SIZE} &
  \multirow{2}{*}{INFERENCE} &
  \multicolumn{3}{c|}{FN} &
  \multicolumn{3}{c|}{LN} \\ \cline{4-9} 
 &
   &
   &
  \multicolumn{1}{c|}{WERR} &
  \multicolumn{1}{c|}{F1} &
  Latency &
  \multicolumn{1}{c|}{WERR} &
  \multicolumn{1}{c|}{F1} &
  Latency \\ \hline
STREAM-BASE &
   &
   &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{71.4} &
  -- &
  \multicolumn{1}{c|}{0.0} &
  \multicolumn{1}{c|}{67.9} &
  -- \\ \hline
\multirow{10}{*}{STREAM-ADAPT} &
  250 &
  \multirow{5}{*}{FULL CATALOG} &
  \multicolumn{1}{c|}{23.9} &
  \multicolumn{1}{c|}{84.2} &
  0.52 &
  \multicolumn{1}{c|}{36.7} &
  \multicolumn{1}{c|}{88.4} &
  0.54 \\ \cline{2-2} \cline{4-9} 
 &
  1000 &
   &
  \multicolumn{1}{c|}{18.1} &
  \multicolumn{1}{c|}{81.1} &
  0.88 &
  \multicolumn{1}{c|}{29.5} &
  \multicolumn{1}{c|}{85.1} &
  0.88 \\ \cline{2-2} \cline{4-9} 
 &
  5000 &
   &
  \multicolumn{1}{c|}{6.4} &
  \multicolumn{1}{c|}{75.6} &
  2.72 &
  \multicolumn{1}{c|}{21.3} &
  \multicolumn{1}{c|}{80.9} &
  2.40 \\ \cline{2-2} \cline{4-9} 
 &
  10000 &
   &
  \multicolumn{1}{c|}{2.1} &
  \multicolumn{1}{c|}{73.4} &
  5.13 &
  \multicolumn{1}{c|}{15.0} &
  \multicolumn{1}{c|}{77.2} &
  4.80 \\ \cline{2-2} \cline{4-9} 
 &
  20000 &
   &
  \multicolumn{1}{c|}{1.1} &
  \multicolumn{1}{c|}{73.0} &
  8.67 &
  \multicolumn{1}{c|}{13.1} &
  \multicolumn{1}{c|}{74.8} &
  8.11 \\ \cline{2-9} 
 &
  250 &
  \multirow{5}{*}{FAISS} &
  \multicolumn{1}{c|}{23.9} &
  \multicolumn{1}{c|}{84.2} &
  0.46 &
  \multicolumn{1}{c|}{36.7} &
  \multicolumn{1}{c|}{88.4} &
  0.45 \\ \cline{2-2} \cline{4-9} 
 &
  1000 &
   &
  \multicolumn{1}{c|}{18.1} &
  \multicolumn{1}{c|}{81.1} &
  0.45 &
  \multicolumn{1}{c|}{30.4} &
  \multicolumn{1}{c|}{85.6} &
  0.59 \\ \cline{2-2} \cline{4-9} 
 &
  5000 &
   &
  \multicolumn{1}{c|}{6.9} &
  \multicolumn{1}{c|}{76.4} &
  0.45 &
  \multicolumn{1}{c|}{22.2} &
  \multicolumn{1}{c|}{81.5} &
  0.46 \\ \cline{2-2} \cline{4-9} 
 &
  10000 &
   &
  \multicolumn{1}{c|}{2.7} &
  \multicolumn{1}{c|}{73.6} &
  0.47 &
  \multicolumn{1}{c|}{15.9} &
  \multicolumn{1}{c|}{77.8} &
  0.49 \\ \cline{2-2} \cline{4-9} 
 &
  20000 &
   &
  \multicolumn{1}{c|}{1.6} &
  \multicolumn{1}{c|}{73.6} &
  0.47 &
  \multicolumn{1}{c|}{14.0} &
  \multicolumn{1}{c|}{75.4} &
  0.47 \\ \hline
\multirow{10}{*}{STREAM-ADAPT-DISC} &
  250 &
  \multirow{5}{*}{FULL CATALOG} &
  \multicolumn{1}{c|}{29.3} &
  \multicolumn{1}{c|}{86.8} &
  0.50 &
  \multicolumn{1}{c|}{38.2} &
  \multicolumn{1}{c|}{89.6} &
  0.58 \\ \cline{2-2} \cline{4-9} 
 &
  1000 &
   &
  \multicolumn{1}{c|}{23.4} &
  \multicolumn{1}{c|}{84.2} &
  0.82 &
  \multicolumn{1}{c|}{32.4} &
  \multicolumn{1}{c|}{87.9} &
  0.78 \\ \cline{2-2} \cline{4-9} 
 &
  5000 &
   &
  \multicolumn{1}{c|}{13.3} &
  \multicolumn{1}{c|}{80.0} &
  2.46 &
  \multicolumn{1}{c|}{15.9} &
  \multicolumn{1}{c|}{81.0} &
  2.84 \\ \cline{2-2} \cline{4-9} 
 &
  10000 &
   &
  \multicolumn{1}{c|}{10.1} &
  \multicolumn{1}{c|}{78.5} &
  4.95 &
  \multicolumn{1}{c|}{15.0} &
  \multicolumn{1}{c|}{78.8} &
  5.10 \\ \cline{2-2} \cline{4-9} 
 &
  20000 &
   &
  \multicolumn{1}{c|}{5.3} &
  \multicolumn{1}{c|}{75.3} &
  8.89 &
  \multicolumn{1}{c|}{13.0} &
  \multicolumn{1}{c|}{77.5} &
  8.12 \\ \cline{2-9} 
 &
  250 &
  \multirow{5}{*}{FAISS} &
  \multicolumn{1}{c|}{29.3} &
  \multicolumn{1}{c|}{86.8} &
  0.46 &
  \multicolumn{1}{c|}{38.2} &
  \multicolumn{1}{c|}{89.6} &
  0.45 \\ \cline{2-2} \cline{4-9} 
 &
  1000 &
   &
  \multicolumn{1}{c|}{23.4} &
  \multicolumn{1}{c|}{84.2} &
  0.46 &
  \multicolumn{1}{c|}{32.4} &
  \multicolumn{1}{c|}{87.9} &
  0.45 \\ \cline{2-2} \cline{4-9} 
 &
  5000 &
   &
  \multicolumn{1}{c|}{13.3} &
  \multicolumn{1}{c|}{79.7} &
  0.50 &
  \multicolumn{1}{c|}{15.9} &
  \multicolumn{1}{c|}{80.8} &
  0.49 \\ \cline{2-2} \cline{4-9} 
 &
  10000 &
   &
  \multicolumn{1}{c|}{10.1} &
  \multicolumn{1}{c|}{78.5} &
  0.45 &
  \multicolumn{1}{c|}{14.0} &
  \multicolumn{1}{c|}{78.5} &
  0.49 \\ \cline{2-2} \cline{4-9} 
 &
  20000 &
   &
  \multicolumn{1}{c|}{5.9} &
  \multicolumn{1}{c|}{75.9} &
  0.48 &
  \multicolumn{1}{c|}{11.6} &
  \multicolumn{1}{c|}{77.8} &
  0.46 \\ \hline
\end{tabular}
\caption{Performance across varying catalog sizes}
\label{tab:my-table}
\end{table*}
